Citrus-V: Advancing Medical Foundation Models with Unified Medical Image Grounding for Clinical Reasoning

Medical imaging provides critical evidence for clinical diagnosis, treatment planning, and surgical decisions, yet most existing imaging models are narrowly focused and require multiple specialized networks, limiting their generalization. Although large-scale language and multimodal models exhibit strong reasoning and multi-task capabilities, real-world clinical applications demand precise visual grounding, multimodal integration, and chain-of-thought reasoning. We introduce Citrus-V, a multimodal medical foundation model that combines image analysis with textual reasoning. The model integrates detection, segmentation, and multimodal chain-of-thought reasoning, enabling pixel-level lesion localization, structured report generation, and physician-like diagnostic inference in a single framework. We propose a novel multimodal training approach and release a curated open-source data suite covering reasoning, detection, segmentation, and document understanding tasks. Evaluations demonstrate that Citrus-V outperforms existing open-source medical models and expert-level imaging systems across multiple benchmarks, delivering a unified pipeline from visual grounding to clinical reasoning and supporting precise lesion quantification, automated reporting, and reliable second opinions.

==> sections/cases.tex <==
\section{Case Studies}
% 检测分割
% 报告生成（多模态思维链推理）
% 医学文档理解（基于化验单的问答）
% QA问答
%  影像问答
%   能否识别左右（与GPT4.1的比较）
%  文本问答
%  影像、化验检查、病史的联合推理
\todo[color=red]{@qintian}
